Signal Formation in Various Detectors

In this write-up we present the general theory of the signal formation in various detectors. We follow a pedagogical analysis and presentation such that the results could be easily understood and applied by the interested reader to the different detector configurations. We include few applications to gaseous detectors, namely, Monitored Drift Tubes (MDT) and micro-pattern gaseous detectors of the Micromegas type.

==> Conclusions.tex <==
\section{Conclusions}
\label{sec:conclusion}


A detailed study of the MM detectors and their performance when operated under the influence of magnetic field has been presented. The drifting of the ionization electrons inside the magnetic field has been simulated and exercised using the H2 test beam superconductive magnet. Test beam results appear to be in line with what we expect from our simulation and the theoretical models.\\

\noindent In order to understand the effect of the magnetic field on the MM and correct for it, the exact values of the drift velocity and the Lorentz angle, that correspond to the specific magnetic field environment of each MM, have to be used. These can either be extracted directly from simulation or can be measured using experimental data. Overall we may conclude that the performance of the MM detector doesn't show any signs of degradation when operating inside a magnetic field.

%A detailed study of the MM detectors and their performance when operated under the influence of magnetic field has been presented. The precise knowledge of the drift velocity 
% and the Lorentz angle due to the magnetic field has been proven to be essential for 
%
% while the results from test beam performance studies appear to be in line with what we expect from our simulation and the theoretical models.
%
%\paragraph{Simulation $\&$ Theoretical Models}
%We have studied the drifting of the electrons in a standard gas mixture Ar:CO$\mathrm{_2}$ 93:7 for all the possible configurations of applied magnetic field and for different values of the electric field applied in the drift region. The magnetic force alters the drifting electrons' trajectory and as a result the drift velocity of these charges strongly depends on the magnetic field. Moreover theoretical calculations have been carried out and we have extracted a simplified model which approximates in macroscopic scale the electron's drifting in magnetic field. 
%
%\paragraph{Test Beam Data Analysis}
%The analysis of the H2 test beam data was mainly focused in understanding the effect of the magnetic field on the MM performance as well as validating our simulation studies. We describe techniques for measuring the electron drift velocity and the Lorentz angle for various magnetic field intensities. Track reconstruction in magnetic field using the MM detector's \textmu TPC mode and we were able to precisely reconstruct the effective track angles with a very good spatial resolution despite any effects of the field. Exploiting also the back to back configuration we have proven that the offsets introduced due to the magnetic field effect can be canceled out combining the data of one MM doublet.\\
%
%
%\noindent Overall we may conclude that the performance of the MM detector doesn't show any signs of degradation when operating inside magnetic field. Using the test beam data we have successfully measured the drift velocity along with the Lorentz and the effective angle for different field values and the results reproduce the values expected from simulation. Our measurement of the spatial resolution is slightly worse than the zero field case but it remains stable along the different values of the magnetic field. This is not due to the presence of the magnetic field, but it is simply due to the fact that in H2 test beam the amplification field applied on the MMs was lower than the nominal. This affects directly the chamber's performance increasing the uncertainty in position measurement.  

==> Introduction.tex <==
\section{Introduction}
\label{sec:introduction}

The micromegas, an abbreviation for MICRO MEsh GAseous Structure (MM), technology was developed in the middle of the 1990's introducing a micropattern gaseous detector with two asymmetric regions\cite{FirstReference}. Standard MM detectors consist of a planar (drift) electrode, a gas gap of a few millimeters thickness acting as conversion and drift region, and a thin metallic mesh at typically $100-150\,$\textmu m distance from the readout electrode, creating the amplification region, as shown in Figure \ref{fig:mm_principle}. The HV potentials are chosen such that the electric field in the drift region is a few hundred V/cm, and 40$-$50 kV/cm in the amplification region achieving gas gain values of the order of $\mathrm{10^4}$. \\

\begin{figure}[H]
\centering
\includegraphics[scale=0.12]{plots/mm_structure}
\includegraphics[scale=0.3]{plots/mm_principle}
\caption{Left: MM detector structure of a standard non resistive MM. chamber Right: Principle of operation for a resistive MM chamber with readout strips of $400\,\upmu \mathrm{m}$ pitch.}  
\label{fig:mm_principle}
\end{figure}

\noindent Charged particles traversing the drift space ionize the gas and the electrons, liberated by the ionization process, drift towards the mesh (in tens of nanoseconds). With an electric field in the amplification region $50-100$ times stronger than the drift field, the mesh is transparent to more than $95\,\%$ of the electrons. The electron avalanche takes place in the thin amplification region in less than a nanosecond, resulting in a fast pulse on the readout strip\cite{ThirdReference}. The drifting of the electrons and the avalanche formation in the amplification region for perpendicular and inclined, with respect to the chamber plane, tracks is illustrated in the right part of Figure \ref{fig:mm_principle}. The ions that are produced in the avalanche process move towards the mesh with velocities about $100$ times smaller than the electrons. 

\begin{figure}[H]
\centering
\includegraphics[scale=0.9]{plots/RMM_structure_side.pdf}
\caption{Spark Resistant MM. Sketch of the resistive and readout strip structure.} 
\label{fig:mm_res}
\end{figure}

\noindent Adding a layer of resistive strips on top of a thin insulator directly above the readout electrode, as shown in Figure \ref{fig:mm_res}, the MM becomes spark-insensitive. The readout electrode is no longer directly exposed to the charge created in the amplification region. The signals on the readout strips are partly induced signals and partly capacitively coupled to it. By adding this protection some fraction of the signal height is lost but the chamber can be operated at higher gas gain because sparking is reduced by about three orders of magnitude\cite{SecondReference}.\\

\noindent The MM technology is quite attractive for High Energy Particle Physics experiments due to its high rate capability, excellent performance and
simplicity of construction. As a result an R$\&$D activity started in 2007, called Muon ATLAS MicroMegas Activity (MAMMA), to explore the potential of the MM
technology for use in LHC experiments. On May 2013 ATLAS decided to equip the New Small Wheel (NSW) with MM detectors\cite{FourthReference}, combining triggering and precision tracking functionality in a single device\cite{JoergReference}.


\begin{figure}[H]
\centering
\includegraphics[scale=0.03]{plots/mm_tb_h2.jpg}
\includegraphics[scale=0.03]{plots/mm_tb_h6.jpg}
\includegraphics[scale=0.04]{plots/mm_tb_desy.jpg}
\includegraphics[scale=0.049]{plots/sw_mm_picture.png}
\caption{MAMMA collaboration various test beam activities including installation in ATLAS (H2, H6, DESY, ATLAS installation).}
\label{fig:mm_tb_h6}
\end{figure}

\noindent Numerous resistive type prototypes of various sizes, and resistivity values have been fabricated over the past years. In addition, a significant amount of time has been invested from the collaboration in testing the operational and performance characteristics of the chambers. Test have been carried out at CERN as well as in other collaborating institutes across Europe with a great number of people being involved. Some photos of the four different setups as well as the chambers installed in the ATLAS cavern are shown in Figure \ref{fig:mm_tb_h6}.\\

\noindent Because of the magnetic field in the ATLAS NSW ($\leq$0.4\,T) region, the study of the MM operated inside a magnetic field has been of particular interest. Such a study has been carried out in the H2 test beam at CERN during June 2012. The effect of the magnetic field on the detector performance is compared to simulation and theoretical expectations based on a simplified model.

%\noindent In addition to analyzing and understanding the test beam data, detailed simulation of the MM chambers has been developed. By comparing the results from data analysis with simulation expectations we were able to finely tune the detectors operational characteristics while, innovative analysis and reconstruction techniques have been developed. Due to the magnetic field in the ATLAS NSW ($\leq$0.4\,T) region, where the MM detector should be able to demonstrate its superb performance characteristics, the study of the MM operated inside a magnetic field has been of particular interest. A dedicated test beam in the H2 CERN north area has been used to study the effect of the field on the detector performance and the results are compared to simulation and to theoretical expectations based on a simplified model.


